The Legacy of Authoritarianism in a Democracy

Recent democratic backsliding and the rise of authoritarian regimes worldwide have rekindled interest in understanding the causes and consequences of such authoritarian rule in democracies. In this paper, I study the long-run political consequences of authoritarianism in the world's largest democracy. Exploiting the unexpected timing of the authoritarian rule imposed in India in the 1970s and using a difference-in-difference (DID), triple difference (DDD), and a regression discontinuity design (RDD) estimation approach, I document a sharp decline in the then-dominant incumbent, the Indian National Congress party's political dominance in subsequent years. I also present evidence that the decline in political dominance was not at the expense of a lower voter turnout rate. Instead, a sharp rise in the number of opposition candidates contesting elections in subsequent years played an important role. Finally, I examine the enduring consequences, revealing that confidence in politicians remains low in states where the draconian policy was high.

==> table/table3b.tex <==
%\documentclass[]{article}
%\setlength{\pdfpagewidth}{8.5in} \setlength{\pdfpageheight}{11in}
%\begin{document}
%\begin{tabular}{lcccccc} \hline
% & (1) & (2) & (3) & (4) & (5) & (6) \\
%VARIABLES &  &  &  &  &  &  \\ \hline





%%%%% include the following
\usepackage[margin=1in]{geometry}
\usepackage{amssymb}
\usepackage{rotating}
\usepackage{caption}
\begin{document}
%%%%% include the following
\clearpage 
\begin{table}[htbp]
\caption{DDD Estimation}
\begin{center}
\resizebox{\linewidth}{!}{%
\begin{tabular}{lcccccc} 
\hline \hline                    \\
                & \multicolumn{5}{c}{All Sample}                            & Major Elections  \\
                & (1)       & (2)       & (3)       & (4)       & (5)       & (6)              \\ 
\hline
 &  &  &  &  &  &  \\



 &  &  &  &  &  &  \\
Post x INC x Excess Sterilization & -0.0328*** & -0.0328*** & -0.0346*** & -0.0345*** & -0.0347*** & -0.0351*** \\
 & (0.00770) & (0.00770) & (0.00899) & (0.00897) & (0.00905) & (0.00917) \\
 &  &  &  &  &  &  \\
Observations & 89,529 & 89,529 & 89,529 & 89,526 & 89,526 & 87,041 \\
R-squared & 0.346 & 0.346 & 0.348 & 0.349 & 0.349 & 0.352 \\
Party FE & \checkmark & \checkmark & \checkmark & \checkmark & \checkmark & \checkmark \\
Year FE & \checkmark & \checkmark & \checkmark & \checkmark & \checkmark & \checkmark \\
Party Type FE & \checkmark & \checkmark & \checkmark & \checkmark & \checkmark & \checkmark \\
State FE & \checkmark & \checkmark & \checkmark &  & \checkmark & \checkmark \\
 Constituency FE &  &  &  & \checkmark & \checkmark & \checkmark \\ \hline
 %%%%%%%%%% Include the following
 \hline \hline
\end{tabular}
}
\end{center}
{Notes: The data are from all general elections to the lower house of the Indian parliament (Lok Sabha) between 1962-2019. The unit of observation is a candidate. Each column reports estimates from OLS regression. Party FE includes the dummy variable of each party from which the candidate is contesting (independent party if the candidate has no party affiliation). Year FE includes election year fixed effects. Party Type FE includes the dummy variable of types of the political party (such as a national, state-based, local party), which proxies for geographical representation of a party. Constituency FE and State FE include the dummy variable of each constituency and state from which the candidate is contesting, respectively. Robust standard errors in parentheses clustered at constituency level. *** p$<0.01$, ** p$<0.05$, * p$<0.1$}
\end{table}











\end{document}

